HouseDiffusion: Vector Floorplan Generation via a Diffusion Model with Discrete and Continuous Denoising

The paper presents a novel approach for vector-floorplan generation via a diffusion model, which denoises 2D coordinates of room/door corners with two inference objectives: 1) a single-step noise as the continuous quantity to precisely invert the continuous forward process; and 2) the final 2D coordinate as the discrete quantity to establish geometric incident relationships such as parallelism, orthogonality, and corner-sharing. Our task is graph-conditioned floorplan generation, a common workflow in floorplan design. We represent a floorplan as 1D polygonal loops, each of which corresponds to a room or a door. Our diffusion model employs a Transformer architecture at the core, which controls the attention masks based on the input graph-constraint and directly generates vector-graphics floorplans via a discrete and continuous denoising process. We have evaluated our approach on RPLAN dataset. The proposed approach makes significant improvements in all the metrics against the state-of-the-art with significant margins, while being capable of generating non-Manhattan structures and controlling the exact number of corners per room. A project website with supplementary video and document is here https://aminshabani.github.io/housediffusion.

==> 2023 CVPR - HouseDiffusion/Sections/0-abstract.tex <==
The paper presents a novel approach for vector-floorplan generation via a diffusion model, which denoises 2D coordinates of room/door corners with two inference objectives: 1) a single-step noise as the continuous quantity to precisely invert the continuous forward process; and 2) the final 2D coordinate as the discrete quantity to establish geometric incident relationships such as parallelism, orthogonality, and corner-sharing.
%
Our task is graph-conditioned floorplan generation, a common workflow in floorplan design. We represent a floorplan as 1D polygonal loops, each of which corresponds to a room or a door.
%in the input constraint graph.
%
Our diffusion model employs a Transformer architecture at the core, which controls the attention masks based on the input graph-constraint and directly generates vector-graphics floorplans via a discrete and continuous denoising process.
%
We have evaluated our approach on RPLAN dataset.
%and.
%compared against the current state-of-the-art. 
The proposed approach makes significant improvements in all the metrics against the state-of-the-art with significant margins, while being capable of generating non-Manhattan structures and controlling the exact number of corners per room. A project website with supplementary video and document is here \href{https://aminshabani.github.io/housediffusion}{https://aminshabani.github.io/housediffusion}.

==> 2023 CVPR - HouseDiffusion/Sections/1-introduction.tex <==
\section{Introduction}
\label{sec:introduction}

Automated floorplan generation made tremendous progress in the last few years.
While not being fully autonomous yet, the state-of-the-art techniques
% While state-of-the-art techniques cannot take into account all complex real-world constraints such as building codes and external/environmental factors, the system
help architects to explore the space of possible designs quickly~\cite{housegan,houseganpp}.
% and make their workflows more efficient~\cite{housegan,houseganpp}. 
90\% of buildings do not have dedicated architects for floorplan design due to their cost in North America. This technology will make the work of professional architects affordable to more house buyers.


%Towards a fully autonomous system or providing more effective assistance, the system needs to produce more realistic, diverse, and compatible (with user constraints) designs.
Despite recent progress, state-of-the-art floorplan generative models produce samples that are incompatible with the input constraint, lack in variations, or do not look like floorplans~\cite{houseganpp}. The issue is the raster geometry analysis via convolutions, where a room is represented as a binary image. The raster analysis is good at local shape refinement but lacks in global reasoning, and requires non-trivial post-processing for vectorization~\cite{floor-sp,houseganpp}.
%
On the other hand, direct generation of vector floorplans is not trivial either.
Different from the generation of images or natural languages, structured geometry exhibit precise incident relationships among architectural components (e.g., doors and rooms). For example, a wall is usually axis-aligned, where the coordinate values of adjacent corners are exactly equal. A wall might be shared with adjacent rooms further.
%
Direct regression of 2D coordinates would never achieve these relationships. 
%A standard application of DMs could regress 2D coordinates of rooms corners but never achieve exact incident relationships. 
One could use a discrete representation such as one hot encoding over possible coordinate values with classification, but this causes a label imbalance (i.e., most values are 0 in the encoding) and fails the network training.


This paper presents a novel approach for graph-constrained floorplan generation that directly generates a vector-graphics floorplan (i.e., without any post-processing), handles non-Manhattan architectures, and makes significant improvements on all the metrics. Concretely, a bubble-diagram is given as a graph, whose nodes are rooms and edges are the door-connections. We represent a floorplan as a set of 1D polygonal loops, each of which corresponds to a room or a door, then generate 2D coordinates of room/door corners (See Fig.~\ref{fig:teaser}).
%generate a floorplan as a set of 1D polygonal loops (i.e., 2D coordinates of room corners), each of which corresponds to a room or a door (See Fig.~\ref{fig:teaser}).
%
The key idea is the use of a Diffusion Model (DM) with a careful design in the 
%representation of the inference/
denoising targets.
%of the denosing process.
Our approach infers 1) a single-step noise amount as a continuous quantity to precisely invert the continuous forward process; and 2) the final 2D coordinate as the discrete quantity to establish incident relationships. The discrete representation after the denoising iterations is the final floorplan model.
%After the denoising iterations, the discrete representation becomes the final floorplan model.

Qualitative and quantitative evaluations show that the proposed system outperforms the existing state-of-the-art, House-GAN++~\cite{houseganpp}, with significant margins, while being end-to-end 
%, runs faster
and capable of generating non-Manhattan floorplans with exact control on the number of corners per room.
%
%Following the state-of-the-art floorplan generative model House-GAN++~\cite{houseganpp}, we use the RPLAN dataset with the same metrics to evaluate the results. The proposed system outperforms House-GAN++ with significant margins in all the metrics.
We will share all our code and models.

==> 2023 CVPR - HouseDiffusion/Sections/2-related-work.tex <==
\section{Related Work}

\mysubsubsection{Floorplan generation}
Generation of 3D buildings and floorplans has been an active area of research from a pre-deep learning era~\cite{bao2013generating, hendrikx2013procedural, ma2014game, muller2006procedural, peng2014computing}.
%Using generative models in the generation of 3D buildings and floorplans backs to before the success of deep learning~\cite{bao2013generating, hendrikx2013procedural, ma2014game, muller2006procedural, peng2014computing}.
The research area has further flourished with the emergence of deep learning.
%The surge of deep learning further flourished the research area
%With the advances in Deep Neural Networks, various approaches have been proposed for automated floorplan generation using DNNs. 
Nauata \etal~\cite{housegan} proposed House-GAN as a graph constrained floorplan generative model via Generative Adversarial Network~\cite{goodfellow2020generative}. House-GAN generates segmentation masks of different rooms and combines them to a single floorplan. The authors further improved the quality of the generation by House-GAN++~\cite{houseganpp}, which iteratively refines a layout.
%as an iterative refinement approach.
%to improve the quality of the generated floorplans. 
%
Given the boundary of a floorplan, Upadhyay \etal~\cite{upadhyay2022flnet} used the embedded input boundary as an additional input feature to predict a floorplan. Hu \etal~\cite{hu2020graph2plan} proposed Graph2Plan that retrieves a graph layout from a dataset and generates room bounding boxes as well as a floorplan in an ad-hoc way.
%to generate a floorplan by retrieving a graph layout from a predefined dataset in an ad-hoc way and using it to generate a set of room bounding boxes and a floorplan raster image that together create the final floorplan.
%
Sun \etal~\cite{sun2022wallplan} proposed to iteratively generate connectivity graphs of rooms and a floorplan semantic segmentation mask.
%a floorplan and 
%inside the boundary along with the floorplan semantic segmentation mask.
%
Given a set of room types and their area sizes as the constraint, Luo and Huang~\cite{luo2022floorplangan} proposed a vector generator and a raster discriminator to train a GAN model using differential rendering. Although their method generates vector floorplans directly, it is limited to rectangular shapes.
%, which highly limits the generated floorplans. 
Along with the adjacency graph as the input, Yin \etal~\cite{bisht2022transforming} use graph-theoretic and linear optimization techniques to generate floorplans.
%a graph optimization method to generate mathematically possible floorplans.
%
Our paper also tackles a graph-constrained floorplan generation with a bubble diagram as the constraint~\cite{houseganpp}.
%We follow the same input constraints as of \cite{houseganpp} on generating a floorplan given an input bubble diagram. 
The key difference is that HouseDiffusion processes a vector geometry representation from start to finish, and hence, directly generating vector floorplan samples.
%works in the vector geometry space
%n vector space,
%it is capable of generating non-manhattan floorplans, and it does not require any post-processing.

% maybe basically housegan houesgan++. and some recent works which were kind of inspired by our papers.
% there is no need to cite many works which housegan/housegan++ cited. This part should not be hard as we know these things.

\mysubsubsection{Diffusion models}
Deep generative models have seen great success in broader domains~\cite{goodfellow2020generative, oord2016wavenet, wang2018pixel2mesh, qi2017pointnet, lim2017enhanced}, where a Diffusion Model (DM)~\cite{sohl2015deep,yang2022diffusion,cao2022survey} is an emerging technique.
%a long history in the successful demonstration of performance in different domains~\cite{goodfellow2020generative, oord2016wavenet, wang2018pixel2mesh, qi2017pointnet, lim2017enhanced}. 
Ho \etal~\cite{ho2020denoising} used a DM to boost image generation quality.
%achieved a significant sample quality on image generation using Diffusion Models~\cite{sohl2015deep}.
Dhariwal and Nichol~\cite{nichol2021improved} made improvements by proposing a new noise schedule and learning the variances of the reverse process.
%learning the variances of the reverse diffusion process.
%~\cite{nichol2021improved} 
%
%In the same direction, Dhariwal and Nichol~\cite{nichol2021improved} improved the quality of the diffusion models by proposing a few modifications, such as a new noise schedule and learning the variances of the reverse diffusion process. 
The same authors made further improvements by novel architecture and classifier guidance~\cite{dhariwal2021diffusionbeats}.
%better sample quality by improving the network architecture and benefiting from classifier guidance.
DMs have been adapted to many other tasks 
%Since then, Diffusion Models has been adapted in several tasks such as 
such as Natural Language Processing~\cite{li2022diffusion}, Image Captioning~\cite{chen2022analog}, Time-Series Forecasting~\cite{tashiro2021csdi}, Text-to-Speech~\cite{kim2022guided, koizumi2022specgrad}, and finally Text-to-Image as seen in the great success of 
%finally the great success of Diffusion Models on Multi-Modal learning such as
DALL-E 2~\cite{ramesh2022hierarchical} and Imagen~\cite{saharia2022photorealistic}.
%further attracted researchers to improve Diffusion model in different directions~\cite{yang2022diffusion, cao2022survey}.


Molecular Conformation Generation~\cite{hoogeboom2022equivariant, luo2021predicting, xu2022geodiff, jing2022torsional} and 3D shape generation~\cite{luo2021diffusion, lyu2021conditional, luo2021score, zhou20213d} are probably the closest to our task.
%Molecular conformation generation is probably the closest to ours
%While still very different, the closest works to ours in diffusion models can be considered as Molecular Conformation Generation~\cite{hoogeboom2022equivariant, luo2021predicting, xu2022geodiff, jing2022torsional} and 3D shape generation~\cite{luo2021diffusion, lyu2021conditional, luo2021score, zhou20213d}. 
%
What makes our task unique and challenging is the precise geometric incident relationships, such as parallelism, orthogonality, and corner-sharing among different components, which continuous coordinate regression would never achieve.
%are never achieved when regressing continuous coordinate values.
%
%Our task is different in nature and instead of generating coordinates in continuous space, we focus on generating precise discrete coordinates for floorplans. 
In this regard, several works use discrete state space~\cite{austin2021structured, campbell2022continuous, hoogeboom2021argmax} or learn an embedding of discrete data~\cite{li2022diffusion, chen2022analog} in the DM formulation.
%to generate discrete values using diffusion models.
However, we found that these pure discrete representations do not train well, probably because the diffusion process is continuous in nature.
In contrast, our formulation simultaneously infers a single-step noise as the continuous quantity and the final 2D coordinate as the discrete quantity, achieving superior generation capabilities (See Sect.~\ref{sec:ablation_studies} for more analysis). To our knowledge, our work is the first in using DMs to generate structured geometry.
%In contrast, we train the model to generate the binary vector representation of the discrete values with the same formulation as in continuous space, similar to AnalogBits by Chen et al.~\cite{chen2022analog}. However, we keep both continuous and discrete space to further improve the training and sampling process. To the best of our knowledge, our work is the first in using Diffusion Models on precise geometric incident relationships.

==> 2023 CVPR - HouseDiffusion/Sections/3-method.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Preliminary}
\label{sec:preliminary}
% \yasu{Very nice intro here. This is exactly how I would start. Only suggestion is that we can shorten the first 5 or 6 lines. People know DM already well. We can probably cut 3 or 4 lines at the start of 3.1 probably.}

% \yasu{If we do not need these formula and contents later, we can significantly shorten this. We do not want reviewers to use up their energy before reaching the exciting stuffs. They get quickly tired and lose energy to read our paper.}
Diffusion models (DMs) denoise a Gaussian noise $x_T$ towards a data sample $x_0$ in $T$ steps, whose training consists of the forward and the reverse processes.
%Diffusion Models are a new type of generative models which can be learned to map a given random sample $x_T$ from a Gaussian distribution to a denoised sample $x_0$ from a data distribution using $T$ steps. 
%There are two phases in training of a diffusion model named as forward and reverse processes.
The forward process takes a data sample $x_0$ and generates a noisy sample $x_t$ at time step $t$ by sampling a Gaussian noise $\epsilon \sim \mathcal{N}(0,\textbf{I})$:
%During the forward process, given a data sample $x_0$ and a time step $t$, we generate a noisy sample from the following distribution:
%\begin{equation}
%    q(x_t|x_0) = \mathcal{N}(x_t;\sqrt{\gamma_t}x_0, (1-\gamma_t)I).
%\end{equation}
%Considering $\epsilon_t$ as a random sample from $\mathcal{N}(0,1)$, we can directly obtain a sample $x_t$:
\begin{equation}
    x_t = \sqrt{\gamma_t}x_0 + \sqrt{(1-\gamma_t)}\epsilon. \label{eq:forward}
\end{equation}
$\gamma_t$ is a noise schedule that gradually changes from 1 to 0.
%a monotonically decreasing value from 1 to 0. 
%
The reverse process starts from a pure Gaussian noise $x_T \sim \mathcal{N}(0,1)$ and learns to denoise a sample step by step until reaching $x_0$, where the denoising process takes $x_t$ and estimates $x_{t-1}$ by inferring $x_{t-1}$, $\epsilon$, or $x_0$~\cite{ho2020denoising}.
%with simple linear algebra in the latter two cases~\cite{ho2020denoising}.
%A simple linear algebra , and calculates $x_{t-1}$ via simple linear algebra in the latter two cases.

%$\mathcal{N}(0,1)$ as $x_T$, and iteratively estimate $x_{t-1}$ until reaching $x_0$. 
%These samples can be used to learn a model that gets $x_t$ as the input and generates one of $\epsilon$, $x_{t-1}$, or $x_0$ as the output. 
%In the backward pass, we generate a sample from the model by starting from $t=T$ and passing a random noise from $\mathcal{N}(0,1)$ as $x_T$, and iteratively estimate $x_{t-1}$ until reaching $x_0$. 

%Ho et al.~\cite{ho2020denoising} proposed a simple regression loss function $\mathcal{L}_{t,x_0,\epsilon} = || \epsilon_\theta(x_t, t) - \epsilon ||^2$, with $\epsilon_\theta(x_t, t)$ as the network prediction for $\epsilon$ respect to the parameters $\theta$, and found that using this loss function and training the model to predict $\epsilon_t$ gets best sample quality on images generation. We borrow the same idea by further infer and apply the loss function on both $\epsilon$ in a continuous representation and $x_0$ in a discrete representation to obtain high quality vector floorplans in the output.

% \yasu{This part feels a bit too slow and there is no need to use an equation to talk about a baseline. Does the following story-line work at the start of this section? After giving a brief intro of DM and three inference targets (as you do now but more briefly), we say that our idea is to infer and apply loss to both delta in a continuous representation and x0 in a discrete representation. Then we give an outline of section 3. We can remove 3.1 and just put this intro without a subsection. Then, problem formulation is 3.1...}
% \begin{equation}
%     \mathcal{L}_t = || \epsilon_\theta(x_t, t) - \epsilon_t ||^2
% \end{equation}
% in which $\epsilon_\theta(x_t, t)$ is the prediction of our model with the parameters $\theta$. 

% In the backward pass, we generate a sample from the model by starting from $t=T$ and passing a random noise from $\mathcal{N}(0,1)$ as $x_T$, and iteratively estimate $x_{t-1}$ using:
% \begin{equation}
%     x_{t-1} = \frac{1}{\sqrt{\alpha_t}}(x_t - \frac{1-\alpha_t}{\sqrt{1-\gamma_t}}\epsilon_\theta(x_t, t))+\sigma_t z
% \end{equation}
% \amin{the above should be revised with adding missing definitions and removing unnecessary parts, I will stop here to focus on other parts and will come back}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{HouseDiffusion}
\begin{figure*}[tb]
    \centering
    \includegraphics[width=\textwidth]{Figures/method_v12.pdf}
    \caption{
    % \yasu{Diffusion process and reverse process are separate but are too close now. We may have some vertical space to push here. Add more margins or use colored rectanglea as the background to clarify that there are 2 separate processes here.}
    The forward process takes the ground-truth floorplan $x_0$ and adds a Gaussian noise to create a noisy floorplan sample $x_t$.
    The reverse process takes 
    % floorplan at t
    a noisy floorplan at time $t$ with a bubble diagram as the condition.
    %
    The process infers the corresponding noise $\Tilde{\epsilon}$ and $\Tilde{x}_0$ in the continuous and the discrete (binary) representations, respectively.
    %(discrete) space. 
    %We train the model using the estimated samples from forward pass and use it to denoise the samples during the backward pass of the diffusion process.}
    }
    \label{fig:method} 
\end{figure*}


% \yasu{I don't know why but the figure is not fully polished.  This is more like a design thing.  \\
% %
% First, make some fonts larger. We use "box with black lines" to represent different things "diffusion model" "diffusion process" "discrete head". We should change the style (shape of rectangle, color of a line, or use fill-in color) to distinguish different types of things.     \\
% %
% Do we need "diffusion process arrow", which seems to be equal to forward process? \\
% %
% I wonder if we can change "DiffusionModel" to a different name. This gives an impression that we just take a DM and put things around to build our system, instead of we are making a new DM model by changing the internals. It seems to better to pitch that this is a new DM model. Can we put transformer or MLP (whatever architecture) there and pitch the whole thing as a new diffusion model? \\
% %
% Our key is "continuous" and "discrete". We have discrete but do not have "continuous" in the figure.  \\
% %
% The location of "input conditions" figure is bad? It should be at the start of an arrow, but it looks different. Maybe it is good to draw bounding boxes for the 3 sub-figures (2 floorplans sub-figures and 1 input condition sub-figure). Use a different style than a black rectangle which we already use to show a network module.
% }

%In this section, we first formulate our problem in \ref{sec:problem_formulation}, and then we explain our input representation in~\ref{sec:polygon_representation}, followed by our network architecture in~\ref{sec:network_architecture}, and finally our approach to obtain the denoised generation in both continuous and discrete way \ref{sec:hybrid_diffusion}.

%\subsection{Problem Formulation}
%\label{sec:problem_formulation}

% \yasu{There is one important point here. It is strange to talk about per-room polygon in the problem formuation. Problem formulatoin could be used by others to compete in the future. one room one polygon representation is a special way which is our method. That is not our problem. Floorplan is a graph, and people do not think of this as multiple polygon loops in general. If we define a task output to be a set of 1d polygon loops, others who might directly output a graph will complain. We have to change things here fundamentally. Maybe I flip-flopped here, but now I feel that it is a bad idea to call this problem formulation. Instead it is our representation instead of the problem formulation.}

% \amin{Input, output, metrics, dataset}

%\yasu{The following could be a good start here. Floorplan is a planar graph consisting of corners and connections which can be represented by a list of corners and their adjacency matrix. However, our task is a graph-constrained generation where rooms are given. Therefore, we represent a floorplan as a set of 1D polygonal loops, one per room.... basitcally, we justify our representation choice because we have a bubble diagram as an input. Our representation is not natural as a general vector floorplan. And we also say that this representation has a challenge of expressing precise geometric relationships vertex-sharing at room boundaries and etc.}\amin{hard to say planar graph as doors have intersection with room boundaries, also I guess maybe it's better not to say a graph as the vertices have coordinates and can not be moved.}

% \yasu{Can you change the story line here? We say that bubble-diagram is the constraint, and we generate a floorplan as a per-room 1D polygonal loop, while ensuring that walls and corners are exactly shared across adjacent rooms... In the current right-up, bubble-diagram comes later and our representation appears strange without understanding the bubble diagram constraint.}



HouseDiffusion solves a graph-constrained floorplan generation problem (See Fig.~\ref{fig:teaser}). The constraint is a bubble diagram, whose nodes are rooms and edges are door connections. A room node is associated with a room type.~\footnote{Room types are ``Kitchen", ``Living-room", ``Bedroom", ``Dining-room", ``Bathroom", ``Study-room", ``Balcony", ``Entrance", ``Storage", and ``Unknown". Door types are ``Interior door" and ``Front door".}

The choice of a data representation is crucial for the success of any generative model. A floorplan is a graph, whose general representation is a set of room-corners and their connections as an adjacency matrix. However, this is not an easy representation to generate with the bubble diagram constraint.
Instead, we represent a floorplan as a set of 1D polygonal loops
% $P=\{P_1, P_2, ..., P_N\}$, 
one for each room/door.
% , that is, for each node/edge of the constraint graph. 
%our approach generates a 1D polygonal loop for each room or door, that is, for each node or edge of the constraint graph (See Fig.~\ref{fig:teaser}).
The challenge is to ensure geometric consistencies among the loops.
%which our denoising neural architecture will address.
For example, room corners and walls must be shared exactly without gaps or overlaps.
%
The section explains our solution, namely, the floorplan representation and the network architecture.


%between adjacent rooms, where room corners and walls must be shared exactly without any gaps or overlaps.


%Although this representation has the challenges of expressing precise geometric relationships, vertex-sharing at room boundaries, etc. We believe that this information can be easily obtained by having a high-quality set of polygons as the floorplan.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Floorplan Representation}
\label{sec:polygon_representation}

%, because the interiors corners are shared by multiple rooms.
%
%A floorplan is a set of corners and connections which can be represented by a list of corners and their adjacency matrix. However, 
%
%our task is a graph-constrained generation where rooms and their types are given. Therefore, we represent a floorplan as a set of 1D polygonal loops, one per room or door. Following~\cite{houseganpp}, we pass a bubble diagram (input graph) as the input including rooms and their types represented by nodes. Connected rooms in the bubble diagram have a door connection to each other in the floorplan. The goal is to generate the polygonal loops corresponding to a floorplan based on the given input bubble diagram as it is shown in Figure~\ref{fig:teaser}.


%For example, corners and walls must be shared exactly without any gaps or overlaps among neighboring rooms.

Let $P=\{P_1, P_2, ..., P_N\}$ denote the set of polygonal loops for each room/door to be generated.
% , where $N$ is the total number of nodes and edges in the constraint graph.
Each loop $P_i$ is defined by a sequence of corners with 2D coordinates:
%A polygonal loop $P_i$ requires the number of its corners for a full specification. We use a simple statistics table given the room-type to pick the number of corners $N_i$:
\begin{equation}
P_i = \{C_{i,1}, C_{i,2}, ..., C_{i,N_i}|C_{i,j}\in \mathcal{R}^2\}.
\end{equation}
% Concretely, we consider each floorplan consisting of a set of polygons $P=\{P_1, P_2, ..., P_N\}$ (including both doors and rooms); and each polygon $P_i$ consisting of a set of $N_i$ corners $C_i=\{c_{i,1}, c_{i,2}, ..., c_{i,N_i}|c_{i,j}\in R^2\}$. The goal is to predict the set of $C_i$ for each room $1<i\leq N$. 
%
% Given the bubble diagram as the input, our model generates a set of polygons, one for each node or edge in the graph. To do so, we first randomly sample the coordinates $c_{i,j}$ of each polygon $P_i$ from a Gaussian distribution $\mathcal{N}(0,1)$ as $x_T$ and iteratively denoise them using the backward process described in subsection~\ref{sec:preliminary}. However, There are two main challenges on representing each node as a polygon: 
$N_i$ denotes the number of corners in $P_i$, which needs to be specified or generated.
% The number of corners $N_i$ for each polygon $P_i$ is not given in the input. To solve this,
A common approach is to set the greatest possible number and let the network decide how many corners to use via output flags.
% decide by using output flags.
However, this significantly increases the representation size and makes training harder and inefficient.
%can be padding corners to a fixed large value and leaving it to the network to learn how many corners it needs to use and mask out the other corners. This approach can increase the diversity of the predictions, but it is also harder to train and significantly increases the total number of corners in a floorplan which costs more computations. 
Instead, we construct a histogram of the number of corners for each room/door type from the training samples, then probabilistically pick $N_i$ where the probabilities are proportional to their histogram counts. This heuristic works well in practice. A user could also directly specify the number of corners to control the room shape complexity.
%and allows users to manually control the room shape complexity.

%for each room type or a door from the training samples. We use a uniform 

%In this regard, we instead create a distribution of the number of corners per each room type during training and use it to randomly select the number of corners during the test time. This way we keep the number of corners as optimal as possible while it also provides additional power to apply geometric conditions like specific floorplans by manually selecting the number of corners (Figure~\ref{fig:manual_corner}).

%where probabilities are proportional to the height of the histogram.

Coordinate values $\{C_{i,j}\}$ are integers in the range of $[0, 255]$. In the forward process, we affinely map the range to $[-1, 1]$ and treat as continuous values to be mixed with the Gaussian noise $\mathcal{N}(0,1)$.
In the reverse process, we also represent a coordinate value as a discrete integer in the binary representation, that is, as 8 binary numbers.

%by 8 numbers in a binary format.


%Each floorplan in the dataset have coordinate values $C_{i,j}$ where $C_{i,j}\in [0, 256]$. We represent each coordinate in two spaces, in continuous space by scaling and shifting the coordinates from $[0, 256]$ to $[-1, 1]$ to have a consistent scale between different steps of diffusion process; and also by mapping each coordinate value from $[0, 256]$ to its binary representation using 8 bits to use in our discrete representation.


% \yasu{Define the coordinate normalization process.}

%shapes and distances. One simple example is putting doors in the middle of two rooms. In the raster space, the pixels belonging to each room are given and the network can simply determine the position of the door while in vector space the network only sees a few corners and it requires to interpolate those values. 

%While passing lines instead of corners can mitigate the problem, how we present lines are also another challenge. To avoid this, we simply interpolate the corners of each polygon and expand each corner with multiple points, increasing the number of features of each corner from 2 to $2\times L$ where $L$ is the new number of points per each corner. Figure~\ref{fig:expand_corners} shows an example of how expanding corners can help to better understanding of the shapes while having minimal computational overhead in the first layer of the network.

% \begin{figure}[tb]
%     \centering
%     \includegraphics[width=\linewidth]{Figures/expanding_points.pdf}
%     \caption{We interpolate the values of corners to add additional points and ease the training by representing the lines. In the above example, $L$ is equal to 3.}
%     \label{fig:expand_corners}
% \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{HouseDiffusion Architecture}
\label{sec:network_architecture}
% \yasu{Don't we have nice message passing structure based on the hiearchy of nodes? I thought that this is a part which we can use an illustration to show something cool instead of just texts, which seems hard to be excited. Do we talk about architecture later, and denoising first? Denoising is more about the last step of the network while architecture is likely the stuffs before the last layer. Isn't the order opposite?}

HouseDiffusion is a diffusion model based architecture.
The forward process follows (\ref{eq:forward}), where $\gamma_t$ is a standard cosine noise schedule~\cite{nichol2021improved}. The reverse process is a Transformer~\cite{vaswani2017attention} based neural network, which takes the floorplan representation at time $t$ and infers the representation at time $t-1$ (See Fig.~\ref{fig:method}). We append a superscript $t$ to denote the floorplan sample at time $t$ (\eg, $P^t_i$ or $C^t_{i,j}$).


%Every room or door corner $C_{i,j}$ is a node in the Transformer. 


\mysubsubsection{Feature embedding}
Given a floorplan sample $\{P^t\}$ at time $t$, every room/door corner $C^t_{i,j}$ becomes a node in the Transformer architecture with a $d (=512)$ dimensional embedding vector $\hat{C}^t_{i,j}$.
We initialize the embedding as
%embedding is initialized by 
%Given a coordinate $C^t_{i,j}$ at time $t$, we build a 128 dimensional embedding vector $\hat{C}^t_{i,j}$ for the corner by merging with the other information:
%Given the time step $t$ and the room type $R_i$, we initialize a node embedding
%
% \yasu{Explain here that we intialize a node embedding as follows. Then, there are two important architecture designs: structured attention masking and discrete and continuous denoising. (Then directly goes to mysubsubsection{structured attendion masking}}
%\begin{equation}
    %\hat{C}^t_{i,j} \leftarrow W_1 \mbox{AU}(C^t_{i,j}) + W_2R_i + W_3 [\mathbf{1}(i), \mathbf{1}(j)] + W_4 t \nonumber
%\end{equation}
\begin{equation}
    \hat{C}^t_{i,j} \leftarrow \mbox{Linear}( [\mbox{AU}(C^t_{i,j}), R_i, \mathbf{1}(i), \mathbf{1}(j), t]) \label{eq:embedding}
\end{equation}
% \yasu{Explain 3 terms one by one by providing full dimensions.}
% 1. AU is augmentation function.
%The first term is an embedding of an augmented corner coordinate.
$\mbox{AU}$ augments the corner coordinate by 1) uniformly sampling $L (=8)$ points along the wall to the next corner; and 2) concatenating the sampled point coordinates. The augmentation helps to reason incident relationships along the walls.
%Passing only the room corners $\{C_{i,j}\}$, it is not easy to reason relationships of adjacent rooms sharing walls and corners exactly. We augment ($\mbox{AU}$) each corner representation $C_{i,j}$ by 
%
%is a $512\times 18$ linear projection matrix.
%With abuse of notation, $C_{i,j}$ denotes the augmented corner %coordinates, whose dimension increases from 2 to $2+ 2L (=18)$. 
$R_i$ is a 25D room-type one hot vector. $\mathbf{1}(\cdot)$ denotes a 32D one-hot vector for a room index $i$ and a corner index $j$.
%he second term takes a concatenation of a 25D room-type one hot vector $R_i$ and the position encodings of a room index $i$ and a corner index $j$, represented as a 32D one-hot vector.
$t$ is a scalar.
%the room type as a one hot vector of dimension 25. PE denotes the position encoding of room index $i$ or corner index $j$ as a one hot vector of dimension 32, and $t$ is a scalar. Brackets represents concatenation in the feature dimension, and $W_1$, $W_2$, and $W_3$ are linear projections to embed each value to the model dimension $d$. 
A linear layer converts the embedding to a 512D vector.

%There are two important architecture designs in our method: structured attention masking and discrete and continuous denoising.



% \yasu{ Having bubble diagram as the input constraint, we use this constraint in two ways. First, as the features along with other inputs to the model. At a time step $t$, we pass the expanded version of noisy coordinates $C^t_{i,j}$, with the input conditions (including time step $t$, room/door types, corner indices, and room indices) as the input to our transformer model. Inside the model, we first embed each part of the input (coordinates and conditions) using a linear layer and pass the concatenation of their outputs to the transformer encoder.}
 
 
\mysubsubsection{Continuous denoising}
%Structured attention masking}
% \yasu{refine to make languages consistent.}
% In addition to the node embedding, we use the input bubble diagram to also manage the flow of information. In each layer of the encoder, we use 3 types of attentions (Figure~\ref{fig:model}) to explicitly enforce different relations between corners including: 1) \textit{Component-wise Self Attention (CSA)}: by masking corners attentions to only attend other corners in the same room/door 2) \textit{Relational Cross Attention (RCA)}: by masking corners to only attend the corners of the connected doors, and 3) \textit{Global Self Attention (GSA)}: as the core attention to make sure the close corners of different rooms can share information. For simplicity, we do not put any condition on the distance of corners while one can limit the GSA to only attend corners within a distance to improve the efficiency.
Embedding vectors $\{\hat{C}^t_{i,j}\}$ will go through attention layers with structured masking (See Fig.~\ref{fig:model}).
%
There are three types of attentions in our attention layer:
%structured attention masks
%with different attention structures.
%a sequence attention layers of three types, which control the attention masks based on the input graph constraint.
%
%In addition to the node embedding, we use the input bubble diagram to also manage the flow of information. In each layer of the encoder, we use 3 types of attentions  to explicitly enforce different relations between corners including:
1) Component-wise Self Attention (CSA), limiting attentions among nodes in the same room or door
%by masking the attention of a corner $C_{i,j}$ to only attend other corners in $P_i$. 
2) Global Self Attention (GSA), a standard self-attention between every pair of corners across all rooms;
%: as the core attention to make sure the close corners of different rooms can share information. 
and 3) Relational Cross Attention (RCA), limiting attentions to from-room-to-door or from-door-to-room that are connected in the constraint graph.
%by masking the attention of $C_{i,j}$ to only attend the corners $C_{i', j'}$ only when one of $P_i$ or $P_{i'}$ is door and $P_i$ is connected to $P_{i'}$. 
%
%For simplicity, we do not put any condition on the distance of corners while one can limit the GSA to only attend corners within a distance to improve the efficiency.add
We learn three sets of key/query/value matrices in each of the attention layer per head, while we use four multi-heads.
%four multi-heads in this attention layer.
The results of the three attentions are summed, followed by a standard Add \& Norm layer. The continuous denoising repeats the block of this attention and Add \& Norm layers four times. At the end, a single linear layer infers noise $\epsilon_{\theta}(C_{i,j}, t)$ at each node.
\begin{figure}[tb]
    \centering
    % \includegraphics[width=\linewidth]{Figures/model.pdf}
    \includegraphics[width=\linewidth]{Figures/model_v5.pdf}
    \caption{Given the input bubble diagram, our model benefits from three attention modules explicitly processing different levels of relations between coordinates. The figure shows how a group of coordinates share information with other groups in each attention module. The black cells represent the masked-out attentions.}
    \label{fig:model} 
    % \vspace{-1cm}
\end{figure}

\mysubsubsection{Discrete denoising}
%\label{sec:hybrid_diffusion}
% \yasu{Is the order of "discrete and continuous denoising" then "housediffusion architecture" natural? Is it better to first talk about rough architecture with a big figure, then explain the core DandC denoising process?}\amin{I thought without describing the discrete and continuous differences it will be confusing to have a discrete head. But now I'm thinking both can work, I will try to update.}
%
% \yasu{This should become shorter. }
Geometric incident relationships (e.g., colinearity, orthogonality, or corner sharing) rarely emerge
%are difficult to come by 
through coordinate regression. For example, two coordinates almost never become the same by regression.
%In contrast with the Raster space that a small error in a pixel value can be easily fixed by thresholding, such an error in a corner's coordinate can result in jagged edges or strange shapes in the vector space and thresholding is not trivial for the generated coordinates. 
% \amin{moved to experiments} To generate discrete values with diffusion models, AnolgBits~\cite{chen2022analog} uses the diffusion formulation to simply predict binary representation of the discrete values, making it possible to apply thresholding on the final predictions of the bits to 0 and 1 and obtain the discrete values. However, doing so can reduce the effect of ``denoising steps'' as the model can cheat after a few steps by simply predicting the values close to 1 as 1 and the values close to 0 as 0 (Please see supplementary for more details). 
Our approach infers coordinates in a discrete form.
%, in particular, as an integer in the binary representation, that is, 8 binary numbers indicating an integer in the range $[0, 255]$.
%an integer in a binary number representation. 
Concretely, after obtaining ${C}^{t-1}_{i,j}$ and ${C}^{0}_{i,j}$ from the continuous denoising process, we affinely map $C^{0}_{i,j}$ back to the range $[0, 255]$, apply rounding, and use an ``int2bit" function~\cite{chen2022analog} to convert to a binary representation, that is, 8-dimensional binary vector.
%
%8 dimensional discrete representation. 
We use a similar formula as formula (\ref{eq:embedding}) to obtain a 512D embedding vector for each corner:
\begin{equation}
    \mbox{Linear}( [\mbox{AU}(C^0_{i,j}), \mbox{int2bit}(C^0_{i,j}), R_i, \mathbf{1}(i), \mathbf{1}(j), t]) \label{eq:embedding2}
\end{equation}
% \yasu{Not clear. what do you mean by   add the binary vector? what is the conditions?}
We pass ${C}^{0}_{i,j}$ as the input to the augmentation and we pass the binary representation obtained by int2bit function along with the conditions to help the network by providing the initial binary representation. We repeat two blocks of attention with structured masking, followed by a linear layer to produce an 8-dimensional vector as $C^0_{i,j}$. During testing, we binary threshold $C^0_{i,j}$ and obtain the integer coordinate. During training, we directly use the values without thresholding for a loss function.




%To solve this, we propose a new scheme utilizing both the continuous space and discrete space together. We consider two parts for our model, the core part is always active during both training and the testing and predicts in continues space, while a discrete head only actives when $t$ is reasonably small and
%% gets the embedded values of input conditions, $t$, $x_t$, and the prediction of continues head, $\epsilon_t$, to 
%predicts the binary representation of $x_0$. To train the discrete head, we found that directly passing the continuous space and training for binary output is hard to train as the network needs to also learn the decimal to binary mapping. Therefore, we first use the prediction of the core model to provide a binary estimation of $x_0$ and we pass that along with $\hat{C}^t_{i,j}$ to the discrete head to predict the final prediction. 


\mysubsubsection{Loss functions}
We train our model end-to-end with the simple L2-norm regression loss by Ho \etal~\cite{ho2020denoising} on both continuous and discrete regressions with the same weight. Concretely, $\epsilon_{\theta}(C_{i,j}, t)$ is compared with the ground-truth noise $\epsilon$ from the forward process. $C^0_{i,j}$ is compared with the ground-truth corner coordinate in binary representation.
The inference of $C^0_{i,j}$ becomes accurate only near the end of the denoising process. Therefore, the discrete branch is used during training only when $t < 20$. At testing, we use the denoised integer coordinates from the discrete branch to pass to the next iteration only when $t < 32$.

%In the early steps of denoising, it is not easy to infer $C^0_{i,j}$ accurately, and the loss on the discrete target is used only in the last 


%reshold, superscript $b$ is notation for binary representation, and $\epsilon_{\theta}(x_t, t)$ and $x_{0, {\theta}}^b(x_t, t)$ are the predictions of the network for $\epsilon$ and $x_0^b$ respect to the network parameters $\theta$.



%\begin{equation}
    %\mathcal{Loss} = || \epsilon_{\theta}(C_{i,j}, t) - \epsilon ||^2 + || C^0_{i,j} - x_0^b ||^2
%\end{equation}

%using simple regression loss for both the continuous denoising result as well as the discrete denoising result:
%For the continuous denoising, we use a simple regression loss by Ho et al.~\cite{ho2020denoising} between $\epsilon$ and the noise predicted by the model. We also borrow the same formulation to train the discrete head by applying a regression loss over the binary representation of $x_0$ and its prediction by the model. The total loss to train our model can be defined as following:
%\begin{equation}
%    \mathcal{L}_{t,x_0,\epsilon}= || \epsilon_{\theta}(x_t, t) - \epsilon ||^2 + \omega|| x_{0, {\theta}}^b(x_t, t) - x_0^b ||^2
%\end{equation}
%where $\omega$ is a binary value which equals to 1 when $t$ is smaller than a threshold, superscript $b$ is notation for binary representation, and $\epsilon_{\theta}(x_t, t)$ and $x_{0, {\theta}}^b(x_t, t)$ are the predictions of the network for $\epsilon$ and $x_0^b$ respect to the network parameters $\theta$.


% $\mathcal{L}_{t,x_0,\epsilon} = || \epsilon_\theta(x_t, t) - \epsilon ||^2$ , with $\epsilon_\theta(x_t, t)$ as the prediction of the model for $\epsilon$ respect to the parameters $\theta$. For the discrete head, we also use a simple loss function $\mathcal{L}_{t,x_0,\epsilon} = || x_{0, \theta}'(x_t, t) - x_0' ||^2$


% Finally, we train our model end-to-end usint two loss functions. For the continuous head, we use a simple regression loss function $\mathcal{L}_{t,x_0,\epsilon} = || \epsilon_\theta(x_t, t) - \epsilon ||^2$ proposed by Ho et al.~\cite{ho2020denoising}, with $\epsilon_\theta(x_t, t)$ as the prediction of the model for $\epsilon$ respect to the parameters $\theta$. For the discrete head, we also use a simple loss function $\mathcal{L}_{t,x_0,\epsilon} = || x_{0, \theta}'(x_t, t) - x_0' ||^2$

% with the core model using a simple regression loss between its output and the binary representation of $x_0$. Ho et al.~\cite{ho2020denoising} proposed , and found that using this loss function and training the model to predict $\epsilon_t$ gets best sample quality on images generation. We borrow the same idea by further infer and apply the loss function on both $\epsilon$ in a continuous representation and $x_0$ in a discrete representation to obtain high quality vector floorplans in the output.

% To obtain descrete values, Ho et al.~\cite{ho2020denoising} proposed ~\amin{TODO}.


==> 2023 CVPR - HouseDiffusion/Sections/4-experiment.tex <==
\section{Experiments}

\begin{figure*}[p]
    \centering
    % I rarely shrink a figure size, but this 1% saves us 1 line.
    \includegraphics[width=1.01\textwidth]{Figures/diversity_comparison_v8.pdf}
    % \vspace{10cm}
    \caption{Generated floorplan samples against House-GAN++~\cite{houseganpp}. See supplementary for more examples. Our results look more diverse and higher quality, where the major issue of House-GAN++ is duplicate or missing rooms, ignoring the input constraint.
%
%Our method generates diverse floorplans while consistently having better quality with the same conditions given in the input graph. On the other hand, the main problems of House-GAN++ on generating multiple masks for a single room or missing a room reduce the performance on generating diverse samples.}
    }
    \label{fig:main_qualitative_results}
\end{figure*}

\begin{figure*}[tb]
    \centering
    \includegraphics[width=\textwidth]{Figures/compatibility_comparison.pdf}
    \caption{HouseDiffusion results are more compatible with the input bubble diagram by ensuring the generation of a single polygonal loop for each room/door.
    %
    %Having a single polygon for each node/edge enables our method to generate more compatible results to the input bubble diagram comparing to the state-of-the-art method.
    {\color{darkgreen} Green }, {\color{darkyellow} Yellow }, and {\color{red} Red} indicate correct, missing, and extraneous connections, respectively.}
    %connection, a missing connection, and an extra connection.}
    \label{fig:compatibility_comparison}
\end{figure*}

We use PyTorch to implement the proposed approach based on a public implementation of Guided-Diffusion~\cite{dhariwal2021diffusionbeats}.~\footnote{\href{https://github.com/openai/guided-diffusion}{https://github.com/openai/guided-diffusion}}
%of our implementation. 
Adam~\cite{kingma2014adam} is the optimizer with decoupled weight decay~\cite{loshchilov2018decoupled} for 250k steps with batch-size of 512 on a single NVIDIA RTX 6000. An initial learning rate is 1e-3.
We divide the learning rate by 10 after every 100k steps.
%We use a transformer including 4 layers with a hidden dimension of 512 for our core model and 2 additional layers for the discrete head. Please see supplementary for the detailed settings of our architecture. 
We set the number of diffusion steps to 1000 (unless otherwise noted) and uniformly sample $t$ during training.

%We also consider the resolution of all images as $256\times 256$ while we generate samples for evaluation or in the continuous to binary mapping which results 8 bits for each value. 



%\mysubsubsection{Baselines}
We compare against other graph-constrained floorplan generative models (House-GAN++~\cite{houseganpp} and House-GAN~\cite{housegan}) and scene-graph constrained image generative models (Ashual \etal~\cite{ashual2019specifying}, and Johnson \etal~\cite{johnson2018image}). House-GAN++ is the current state-of-the-art for the task.

%House-GAN++~\cite{houseganpp}, House-

%consider House-GAN++~\cite{houseganpp} as the current state-of-the-art as our main baseline, while we also compare our main experiment with the results of House-GAN~\cite{housegan}, Ashual et al.~\cite{ashual2019specifying}, and Johnson et al.~\cite{johnson2018image} as scene generation methods based on graphs.


We use 60,000 vector floorplans from RPLAN~\cite{rplan} dataset,
%including 60k floorplans in vector format
and the same pre-processing steps as in House-GAN++, where floorplan images have a resolution of $256\times 256$.
%There are 12 room types (Kitchen, Living room, Bedroom, Dining Room, Bathroom, Study room, Balcony, Entrance, Storage, Front and Inner door, and Unknown).
%Each floorplan is also assigned a bubble diagram including room connections and their types.
We divide the floorplan samples into four groups based on the number of rooms (i.e., 5, 6, 7, or 8 rooms). For generating floorplans in each group, we exclude samples in the group from the training so that methods cannot simply memorize samples.
%remaining one.
%based on the number of rooms to four groups with 5, 6, 7, and 8 rooms. For each experiment, we train the method on 3 groups and test on the other group. 
Following House-GAN++, the same three metrics are used for evaluations: Diversity, Compatibility, and Realism. Diversity is the Frechet Inception Distance (FID)~\cite{fid}.
% as the default metric for state-of-the-art generative modeling works capturing both diversity and fidelity.
Compatibility is the modified Graph Edit Distance~\cite{ged} between the input bubble diagram and the one reconstructed from the generated floorplan. Realism is based on user studies (See Section~\ref{sec:main_results} for more details).



To verify the capability of non-Manhattan floorplan generation,
% To verify the effectiveness of our model on the generation of non-manhattan floorplans, 
we create a new benchmark ``Non-Manhattan-RPLAN'' based on RPLAN by randomly adding two corners to an outer wall.
% of floorplans in RPlan dataset to provide non-manhattan parts. 
See supplementary for more details.
%and non-Manhattan floorplan samples.




%\mysubsubsection{Datasets}


%\mysubsubsection{Metrics}
%Following House-GAN++, three metrics are used for evaluations:
%compare our method with the baselines including 

%%%%%%
%\mysubsubsection{Implementation Details}
%Finally, we fix $L$ to 8 as the default value in all of our experiments.

%\amin{MODIFIED UP TO HERE}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Quantitative Evaluations}
\label{sec:main_results}
Table~\ref{tab:main_results} shows the main quantitative evaluations.
% comparison with the baselines. 
For existing methods, we copy the numbers reported in the House-GAN++ paper~\cite{houseganpp}. For the Realism, their paper shows the average score against all the other methods, while we use the score against just the ground-truth, because comparisons between weaker baselines do not provide useful information.
%ompeting methods on the original RPLAN, we use the numbers reported in the House-GAN++ paper~\cite{houseganpp} except the Realism score which
%in which we only consider the users rating on comparing the baseline with ground truth to avoid averaging with weaker baselines. 
Our system, HouseDiffusion, consistently outperforms all the previous methods in all the metrics. Compared to the current state-of-the-art House-GAN++~\cite{houseganpp}, HouseDiffusion makes an average improvement of $67\%$ in diversity and $32\%$ in compatibility.
We also make significant improvements in realism, which we discuss next in detail.
%Furthermore, the generated houses with our method are more than $50\%$ less distinguishable from the ground truth comparing with the House-GAN++. In the next part we discuss the Realism Score in more details.
For non-manhattan RPLAN dataset, HouseDiffusion also makes significant improvements in diversity and compatibility, where House-GAN++ cannot handle non-manhattan structures. The realism score is not used, because the non-manhattan structures were added by heuristics and even the ground-truth may not look realistic.
%ur model gets roughly the same results while Diversity significantly increases for House-GAN++ showing its weakness on generation of non-manhattan floorplans.

\input{2023 CVPR - HouseDiffusion/Tables/main_results}

%%%%%%

%\mysubsubsection{Realism Score}
%\label{sec:pairwise_comparison}
We follow the same process as in House-GAN++ to obtain the realism scores.
We generate 1000 floorplan samples by each system, present two samples (from different systems) to a participant, and ask to choose ``A is better'', ``B is better'', or ``both are equal''.
A method ``A'' earns +1, -1, or 0 point with the above answers, respectively.
%We show the participants a random pair selected from 1000 generated samples of each method (Showing anonymously with method names A and B) and they select one of the three options  In total, each pair of methods has been rated 150 times by participants.
Each pair of systems are evaluated 150 times by 10 participants (i.e., 15 times by each participant).
%In order to obtain the Realism score between our method and ground truth, we followed the same user-study as in ~\cite{houseganpp} with gathering the ratings of 10 participant and asking them to rate 45 pairs of images including 15 pairs on each set of (House-GAN++, HouseDiffusion), (House-GAN++, Ground Truth), and (HouseDiffusion, Ground Truth). 
Table~\ref{tab:main_results} shows the average realism score of each system against the ground-truth. Table~\ref{tab:pairwise comparison} shows the direct comparisons between House-GAN++, HouseDiffusion, and the ground-truth.
%
%
% Comparing the results of (House-GAN++, Ground Truth) pair in our user-study with the one reported in \cite{houseganpp}, we found that our users are more strict than the one in \cite{houseganpp}. We believe that the reason is due to only showing high quality methods in our experiments to participants, making the participants consider stricter rules to distinguish between methods. Although we still report the best number reported in \cite{houseganpp} in Table~\ref{tab:main_results}\amin{This sentence needs to be replaced but I can not think of any yet}.
Both tables show that HouseDiffusion achieves significant improvements with a score of $-0.19$ even against the ground-truth, which is very good.
%considering that the best score would be $0.0$.
The number implies that participants
%
choose our result to be as realistic as the Ground-Truth (``both are equal'') for $81\%$ of the time (assuming they either preferred Ground-Truth or chose equal).
% choose our result to be more realistic than the ground-truth roughly $35\%$ of the time (i.e., $0.19 \approx 0.65 - 0.35$), where the best case is $50\%$ with the score of $0.0$.}
%choose our result to be as realistic as the ground-truth roughly $81\%$ of the times. 
Note that House-GAN++ paper reports $-0.18$ for their best configuration against the ground-truth, but this variant (denoted as ``Ours static*'') requires expensive post-processing~\cite{floor-sp} and filters out incompatible samples based on the ground-truth bubble-diagram that account for 90\% of the generated samples. Our results are direct outputs from our network architecture.
%choose our result to be more realistic than the ground-truth roughly $35\%$ of the time (i.e., $0.19 \approx 0.65 - 0.35$), which is very good considering that the best score would be $0.0$. Note that House-GAN++ paper reports $-0.18$ for their best configuration against the ground-truth, but this variant (denoted as ``Ours static*'') requires expensive post-processing~\cite{floor-sp} and filters out incompatible samples before evaluation based on the ground-truth bubble-diagram that account for 90\% of the generated samples. Our results are direct outputs from our network architecture.

\input{Tables/realism_score.tex}


%\begin{figure}[h]
%    \centering
%    \includegraphics[width=0.7\linewidth]{Figures/pairwise_comparison.pdf}
%    \caption{Our method achieves a significant score of 0.71 in the rating of participant comparing with the current state-of-the-art, showing that the participants choose the floorplans generated by our method over the generated floorplans of House-GAN++~\cite{houseganpp} in $0.71\%$ of the times.}
%    \label{fig:pairwise comparison}
%\end{figure}

\subsection{Qualitative Evaluations}
Figure~\ref{fig:main_qualitative_results} qualitatively compares HouseDiffusion with House-GAN++ by two generated floorplans per bubble-diagram in both Manhattan and Non-Manhattan cases. Please refer to the supplementary for more examples and the supplementary video for the animations of the denoising process.
%shows the comparison of 5 random floorplans generated by our method with the ones generated by House-GAN++ for 2 given input bubble diagrams 
%(See supplementary for more examples). 
%
HouseDiffusion consistently generates higher-quality samples. The major issue of Housen-GAN++ is that the system tends to miss or generate too many rooms, ignoring the input bubble-diagram constraint. For example, the top example in Fig.~\ref{fig:main_qualitative_results} should have one living-room (red), two bedrooms (yellow), and one study (orange), but House-GAN++ makes errors in every single sample. The issue is also highlighted in
%
%House-GAN++~\cite{houseganpp} generates masks for each node which can cause more than one room per node (non-connected masks) or completely missing a node (empty mask); however, our method guarantees one and only one polygon for each node or edge, avoiding those problems. 
%In addition, predicted masks by House-GAN++ can create artifacts which is also not happening in our vectorized format.
%The two aformentioned problems (missing rooms and duplicate rooms) also affect the compatibility of the generated floorplans by House-GAN++, while our method generates more reliable floorplans to the input constraint, 
Fig.~\ref{fig:compatibility_comparison}, which visualizes the bubble-diagrams of generated floorplan samples.
%show the estimated bubble diagram of floorplans generated by both methods comparing to the input diagram.
HouseDiffusion guarantees exactly the correct set of rooms in the output and produces clean wall structures without artifacts (e.g., jagged boundaries) thanks to the vector representation.



==> 2023 CVPR - HouseDiffusion/Sections/5-ablation-studies.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Ablation Studies}
\label{sec:ablation_studies}

We conduct a series of ablation studies to verify the effectiveness of our technical contributions and provide an in-depth analysis of our system.
%Some studies are presented in the supplementary due to space limitations.

\mysubsubsection{Discrete and continuous denoising} 
%
To verify the effectiveness of our discrete and continuous denoising scheme, we compare with a recent work AnalogBits~\cite{chen2022analog}, which employs a binary representation to generate discrete numeric values in a diffusion model framework.
%uses the diffusion formulation to simply predict binary representation of the discrete values, making it possible to apply thresholding on the final predictions of the bits to 0 and 1 and obtain the discrete values.  
%conduct two additional experiments, one with only using continuous space and another experiment with only using binary representation similar to AnalogBits. 
%To generate discrete values with diffusion models, AnolgBits~\cite{chen2022analog}
%However, doing so can reduce the effect of ``denoising steps'' as the model can cheat after a few steps by simply predicting the values close to 1 as 1 and the values close to 0 as 0 (Please see supplementary for more details).
We also create HouseDiffusion only with continuous denoising by simply dropping the discrete branch/loss.
%without the discrete branch/loss, while keeping the rest the same.
Table~\ref{tab:diffusion_domain} demonstrates that the proposed discrete and continuous denoising significantly improves the diversity with a small sacrifice on the compatibility. 
We hypothesize that AnalogBits merely learns the rounding with the binary representation alone when $t$ is small, which reduces the generation quality.
%, we hypothesis that when $t$ is relatively small by using a binary representation alone, the network 
%learns a simple mapping of $f:x_t\rightarrow \lfloor x_t+\frac{1}{2} \rfloor$ instead of the dataset distribution which reduces the final quality of the generated samples.
%
%Comparing with AnalogBits, we hypothesis that when $t$ is relatively small by using a binary representation alone, the network learns a simple mapping of $f:x_t\rightarrow \lfloor x_t+\frac{1}{2} \rfloor$ instead of the dataset distribution which reduces the final quality of the generated samples.

%\yasu{Do you have anything here? The original text did not make much sense to me here.}

%shows the diversity and compatibility of each paradigm. Although AnalogBits have better Diversity than than training in Continues space, it significantly has worse compatibility score. Our HybridDiffusion gets the best results on both Diversity and Compatibility showing the effectiveness of our method.
%
%For continues space we simply remove the discretization head of our model while keeping other parts the same. For training our model in binary space, we again remove the discretization head and we follow the training scheme of AnalogBits. 

\input{2023 CVPR - HouseDiffusion/Tables/diffusion_domain}
%%%%%%

\mysubsubsection{Attention modules}
HouseDiffusion employs three different types of attentions.
%We benefit from 3 different attention modules in our network architecture to enforce different relations between corners.
Table~\ref{tab:different_attentions} and Fig.~\ref{fig:attention_modules} qualitatively and quantitatively measure their effectiveness by dropping the three attentions one by one.
%drop each of the three attentions, qualitatively and quantitatively measuring the performance drop.
%drop each of the three attentions, qualitatively and quantitatively measuring the performance drop.
%shows the effect of removing each attention in the final result. As it is expected, 
Global Self Attention (GSA) has the highest impact on realism (qualitatively in Fig.~\ref{fig:attention_modules}) and diversity as expected, because this accounts for the attentions between every pair of nodes.
%final result and training the model without this attention can reduce the capability of the corners to see their surroundings and result in lower quality floorplans. 
%
Relational Cross Attention (RCA) enforces connections between rooms and doors and has the most impact on the compatibility metric.
%each room and its connected doors and removing it will highly reduce the compatibility score. 
Component-wise Self Attention (CSA) focuses on individual rooms and reveals a significant impact on the room shape quality in Fig.~\ref{fig:attention_modules}, causing self-intersections and ``impossible" shapes without it.
The second last row of Table~\ref{tab:different_attentions} is a version with three times more GSA attention layers instead of the combination of CSA, GSA, and RCA, which demonstrates the importance of using all the attention types.
%, while contributing to both diversity and compatibility.
%provides the explicit connection between corners of each polygon. It helps both in compatibility and diversity by helping the network to easily share information between corners of each polygon and avoid possible overlaps with other polygons. 
%Please see r for additional results on attention modules.

\input{2023 CVPR - HouseDiffusion/Tables/different_attentions}
\begin{figure}[tb]
    \centering
    \includegraphics[width=\linewidth]{Figures/attention_modules.pdf}
    \caption{Qualitative evaluation of the three attention mechanisms. The shape quality degrades significantly in the absence of CSA or GSA. Door placements become corrupted in the absence of RCA.
%RCA accounts for the room-door connections, where the door placements become corrupted while room shapes remain good.
%By removing different attention modules during the test time, we can see the information that each of them convey.
}
    \label{fig:attention_modules}
\end{figure}


%\mysubsubsection{Additonal experiment on attention modules}
%To further demonstrate the effect of each attention module, we trained a network using all three attentions and removed one of them each time during testing. As we can see in Figure~\ref{fig:attention_modules}, with skipping the information of the Relational Self Attention, the rooms get overlapped with each other while the doors will be all positioned in the center. While removing the other two modules will reduce the overall quality of the generation results significantly, we can still observe that removing Global Self Attention cause more overlap and removing Component-wise Self Attention reduce the quality of each room.

%%%%%%

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{Figures/manual_corner_v2.pdf}
    \caption{HouseDiffusion allows us to specify the number of corners per room.
    %By explicitly providing the number of corners, we control the complexity of some room shapes. 
    In this above examples, we increase the number of corners for the dining-room (red room), while keeping all the other rooms to have 4 corners.
    %fix all the rooms to have 4 corners while increasing the number of corners for the dining-room.}
    }
    \label{fig:manual_corner}
\end{figure*}

%%%%%%%%
\mysubsubsection{Geometry modification}
Figure~\ref{fig:manual_corner} demonstrates a new capability of HouseDiffusion, allowing us to specify the exact number of corners per room,
%and hence the complexity of each room shape, 
which is not possible by a raster-based system such as House-GAN++. The figure shows that HouseDiffusion generates floorplans with increasingly more complex dining-room, where the surrounding rooms change their layouts to be consistent.
%the number of corners of a dining room which also adjusts the surrounding rooms to be 
%A new capability of HouseDiffusion is that 
%One of the benefits of using the vectorized floorplan generation is that we can directly apply geometric conditions on the predictions which is not easily available on the Raster space. In order to show this we manually increase the number of corners per dining hall in our input while using a same graph. Figure~\ref{fig:manual_corner} show the results.
%%%%%%


%%%%%%
\mysubsubsection{Discrete steps}
Having both discrete and continuous denoising branches is essential for generating high-quality floorplans, while
%in vector space, while
%. During training, $C^t_{i,j}$ is generated directly from $C^0_{i,j}$, where the discrete branch is less sensitive to the 
%nd the training of discrete head is less sensitive to $t$. To have a smooth training, we limit it to only when $t<20$. However, during the generation, considering that the prediction in each step will be used in the next step, it will be cruciall to use the discrete head properly. 
%In our experiments,
the discrete branch is active in the last 32 iterations at test time.
%when generating floorplan samples.
%$t < 32$ during generatio.
%
We vary this hyperparameter and measure the performance change in Fig.~\ref{fig:discrete_steps}.
%On the other hand, activating the discrete head to predict $x_0$ in step $t$ when $t$ is close to $T$ does not make sense. Therefore, finding the optimal $t$ to activate and use discrete head is an hyperparameter which needs to be tuned. 
%shows the evaluation metrics based on how many steps we use the discrete head at the end of backward process. 
%Continuous means when we only use the continuous head. 
%The amount of discrete denoising have interesting impacts on the compatibility and the diversity metrics.
Limiting to fewer iterations reduces the opportunities of discrete analysis and harms performance. On the other hand, activating the discrete branch too early also degrades the performance, because the discrete analysis is on the final floorplan shape at time 0, whose inference is not accurate at early iterations.
%too many have negative impacts as the inference of the final shape is not easy at the early phase of denoising
%Decreasing the use of the discrete branch to a fewer steps 
%
%Using the discrete branch only for a few steps gives the network less opportunity to denoise the coordinates while using it early can cause discretizing information which can be used in denoising steps.
%
We found that 32 is a good number overall, which is used throughout our experiments.
%works best and we use it for all the experiments. 
% \input{Tables/discrete_steps}
\begin{figure}[tb]
    \centering
    \includegraphics[width=\linewidth]{Figures/steps_table.pdf}
    \caption{
    % \yasu{change "Number of Discrete Steps" to "When to activate the discrete branch (t)"?}
    % \yasu{maybe, we can make this horizontal instead of vertical? I do not like the use of "Step" so many times which seem wasteful and large dead margins at the left and right.  Use abbreviation form for Diversity - Diver.   Compatibility - Compat.   Can you try making this horizontal and use double column table? We could drop 900 step case?  Typo: continues -> Continuous} 
    Using discrete head in a few steps gives less opportunity to the network to refine the discrete coordinates, while using it early can also lead to removing necessarily continuous informations. We fix discrete head to activate when $t<32$.}
    \label{fig:discrete_steps}
\end{figure}
%%%%%%


\mysubsubsection{Corner augmentation}
%Following Subsection~\ref{sec:polygon_representation}, we compare the results obtained by augmenting corners before passing to the model versus passing the corners without augmentation. 
Table~\ref{tab:input_representation} shows the corner augmentation effects in the feature embedding (\ref{eq:embedding}).
While both the diversity and compatibility improve,
% by using corner augmentation, 
the effect is higher for compatibility where the augmented points on the walls enable better analysis of geometric incident relationships.
%further shows the effect of corner augmentation on enabling network to interpolate the correct position of the doors.

% \yasu{This was the same as the other ablation study paragraph, but it should start by referring to what was already explained. This part starts talking about something potentially new. Change the start so that it refers to study the coordinate augmentation in the embedding definition...}
% Having a single point per each corner makes it hard for the network to predict the exact locations of the doors,
%(See Figure~\ref{fig:expand_corners})
% on the other hand, representation of a line is not straight forward, therefore, we simply represent each line with using multiple points. Table~\ref{tab:input_representation} shows the effect of the expanding points. We expand each point in its feature dimension to keep the number of total nodes for the transformer the same and avoid additional heavy computational costs.
\input{2023 CVPR - HouseDiffusion/Tables/input_representation}




==> 2023 CVPR - HouseDiffusion/Sections/6-conclusion.tex <==
\section{Conclusion}
This paper presents a novel floorplan generative model that directly generates vector-graphics floorplans. The approach uses a Diffusion Model with a Transformer network module at the core, which denoises 2D pixel coordinates both in discrete and continuous numeric representations. The discrete representation ensures precise geometric incident relationships among rooms and doors. The transformer module has three types of attentions that exploit the structural relationships of architectural components.
Qualitative and quantitative evaluations demonstrate that the proposed system makes significant improvements over the current state-of-the-art with large margins in all the metrics, while boasting new capabilities such as the generation of non-Manhattan structures or the exact specification of the number of corners. This paper is the first compelling method to directly generate vector-graphics structured geometry.
%that are extremely compact. 
Our future work is the handling of large-scale buildings. We will share all our code and models.



%the system does not take into account complex real-world constraints (e.g., building codes, external/environmental effects, 


==> 2023 CVPR - HouseDiffusion/Tables/discrete_steps.tex <==
\begin{table}[tb]
\caption{\yasu{maybe, we can make this horizontal instead of vertical? I do not like the use of "Step" so many times which seem wasteful and large dead margins at the left and right.  Use abbreviation form for Diversity - Diver.   Compatibility - Compat.   Can you try making this horizontal and use double column table? We could drop 900 step case?  Typo: continues -> Continuous} Using discrete head in a few steps gives less opportunity to the network to refine the discrete coordinates, while using it early can also lead to removing necessarily continuous informations. We fix discrete head to activate when $t<32$.}
% \yasu{Maybe this is better as a bar graph or a graph instead of a table}
% \amin{Due to the scale of numbers, it's hard to show the pattern in a graph or bar, I couldn't create a good visualization yet}
\label{tab:discrete_steps}
\centering
\setlength{\tabcolsep}{3pt}
\small
\scalebox{1.}{\begin{tabular}{c|c|c}
\toprule
   Discrete steps & Diversity $(\downarrow)$ & Compatibility $(\downarrow)$\\
    %
    \cmidrule(lr){1-1}\cmidrule(lr){2-2} \cmidrule(lr){3-3}
    %
    Continues & 38.8\scalebox{0.8}{$\pm$0.9} & 2.2\scalebox{0.8}{$\pm$0.03} \\
    \midrule
    1 Step & 20.8\scalebox{0.8}{$\pm$0.3} & 3.2\scalebox{0.8}{$\pm$0.05}\\
    \midrule
    2 Step & 14.7\scalebox{0.8}{$\pm$0.6} & 3.2\scalebox{0.8}{$\pm$0.04}\\
    \midrule
    4 Step & 9.8\scalebox{0.8}{$\pm$0.2} & 3.2\scalebox{0.8}{$\pm$0.05}\\
    \midrule
    8 Step & 9.3\scalebox{0.8}{$\pm$0.2} & 3.0\scalebox{0.8}{$\pm$0.03}\\
    \midrule
    16 Step & 9.5\scalebox{0.8}{$\pm$0.1} & 2.7\scalebox{0.8}{$\pm$0.07}\\
    \midrule
    32 Step & 9.5\scalebox{0.8}{$\pm$0.1} & 2.5\scalebox{0.8}{$\pm$0.04}\\
    \midrule
    64 Step & 9.6\scalebox{0.8}{$\pm$0.2} & 2.5\scalebox{0.8}{$\pm$0.04}\\
    \midrule
    128 Step & 9.6\scalebox{0.8}{$\pm$0.1} & 2.5\scalebox{0.8}{$\pm$0.02}\\
    \midrule
    256 Step & 9.7\scalebox{0.8}{$\pm$0.3} & 2.6\scalebox{0.8}{$\pm$0.04}\\
    \midrule
    512 Step & 9.6\scalebox{0.8}{$\pm$0.2} & 2.5\scalebox{0.8}{$\pm$0.02}\\
    \midrule
    900 step & 9.8\scalebox{0.8}{$\pm$0.4} & 2.6\scalebox{0.8}{$\pm$0.05} \\
    \bottomrule
\end{tabular}}
\end{table}

==> 2023 CVPR - HouseDiffusion/Tables/dm_params.tex <==
\begin{table}[tb]
\caption{Results of hyper-parameter tuning on the number of steps and noise schedule for our diffusion model. We fix our experiments to 1000 steps with cosine noise schedule~\cite{nichol2021improved}.}
\label{tab:dm_params}
% \vspace{-0.9em}
\centering
\setlength{\tabcolsep}{3pt}
\small
\scalebox{.95}{\begin{tabular}{c|c|c|c}
\toprule
   Noise Schedule & Number of steps & Diversity $(\downarrow)$ & Compatibility $(\downarrow)$\\
    %
    \cmidrule(lr){1-1}\cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4}
    %
    \multirow{1}{*}{Linear}
    & 1000 & 10.5\scalebox{0.8}{$\pm$0.1} & 2.7\scalebox{0.8}{$\pm$0.04}\\
    \midrule
    \multirow{3}{*}{Cosine}
    & 100 & 19.0\scalebox{0.8}{$\pm$0.8} & 3.1\scalebox{0.8}{$\pm$0.0}\\
    & 1000 & 9.5\scalebox{0.8}{$\pm$0.1} & 2.5\scalebox{0.8}{$\pm$0.0}\\
    & 4000 & 12.0\scalebox{0.8}{$\pm$0.3} & 3.2\scalebox{0.8}{$\pm$0.03}\\
    \bottomrule
\end{tabular}}
\end{table}

==> 2023 CVPR - HouseDiffusion/Tables/output_value.tex <==
\begin{table}[b]
\caption{Training the network to predict $\epsilon$ works better in our task comparing with $x_0$ as the output of the model in each step.}
\vspace{-1em}
\label{tab:output_value}
\centering
\setlength{\tabcolsep}{3pt}
\small
\scalebox{1.}{\begin{tabular}{c|c|c}
\toprule
   Network's output & Diversity $(\downarrow)$ & Compatibility $(\downarrow)$\\
    %
    \cmidrule(lr){1-1}\cmidrule(lr){2-2} \cmidrule(lr){3-3}
    %
    $x_0$ & 121.2\scalebox{0.8}{$\pm$1.9} & 4.2\scalebox{0.8}{$\pm$0.0} \\
    \midrule
    $\epsilon$ & 38.8\scalebox{0.8}{$\pm$0.9} & 2.2\scalebox{0.8}{$\pm$0.0}\\
    \bottomrule
\end{tabular}}
\end{table}

==> 2023 CVPR - HouseDiffusion/Tables/realism_score.tex <==
\begin{table}[tb]
\caption{Realism scores among House-GAN++, ours, and the ground-truth.
Our method achieves 0.71 against House-GAN++,
%in comparison with the current state-of-the-art, 
indicating that the participants choose ours to be more realistic
%the floorplans generated by our method over the generated floorplans of House-GAN++~\cite{houseganpp} in $0.71\%$ of the times.
$85\%$ of the times (i.e., $0.71 \approx 0.85 - 0.15$).
}
\label{tab:pairwise comparison}
\centering
\setlength{\tabcolsep}{3pt}
\small
\scalebox{1.}{\begin{tabular}{c|c|c|c}
\toprule
    & House-GAN++ & Ours & Ground Truth\\
    %
    \cmidrule(lr){1-1}\cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4}
    %
    House-GAN++~\cite{houseganpp} & --- & -0.71 & -0.87\\
    \midrule
    Ours & 0.71 & --- & -0.19 \\
    \midrule
    Ground Truth & 0.87 &  0.19 & ---\\
    \bottomrule
\end{tabular}}
\end{table}

==> Tables/different_attentions.tex <==
% \begin{table}[tb]
% \caption{The effect of removing each attention module on the final performance. \yasu{In the figure, orders are csa gsa and rca. Make them the same order here.}}
% \label{tab:different_attentions}
% \centering
% \setlength{\tabcolsep}{3pt}
% \small
% \scalebox{.90}{\begin{tabular}{c|c|c|c|c}
% \toprule
%   CSA & RCA & GSA & Diversity $(\downarrow)$ & Compatibility $(\downarrow)$\\
%     %
%     \cmidrule(lr){1-1}\cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5}
%     %
%           & \cmark & \cmark & 9.9\scalebox{0.8}{$\pm$0.1} & 2.9\scalebox{0.8}{$\pm$0.0} \\
%     \midrule
%     \cmark &        & \cmark & 11.4\scalebox{0.8}{$\pm$0.2} & 6.8\scalebox{0.8}{$\pm$0.0} \\
%     \midrule
%     \cmark & \cmark &        & 12.8\scalebox{0.8}{$\pm$0.2} & 4.0\scalebox{0.8}{$\pm$0.0} \\
%     \midrule
%     \cmark & \cmark & \cmark & \textbf{9.5}\scalebox{0.8}{$\pm$0.1} & \textbf{2.5}\scalebox{0.8}{$\pm$0.0} \\
%     \bottomrule
% \end{tabular}}
% \end{table}

\begin{table}[tb]
\caption{Quantitative evaluation of the three attention mechanisms. The second last row triples the number of GSA layers instead of the combination of CSA, GSA, and RCA.
}
%Ablation study on three attention mechanisms.}
\label{tab:different_attentions}
\centering
\setlength{\tabcolsep}{3pt}
\small
\scalebox{.90}{\begin{tabular}{c|c|c|c|c}
\toprule
   CSA & GSA & RCA & Diversity $(\downarrow)$ & Compatibility $(\downarrow)$\\
    %
    \cmidrule(lr){1-1}\cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4} \cmidrule(lr){5-5}
    %
           & \cmark & \cmark & 9.9\scalebox{0.8}{$\pm$0.1} & 2.9\scalebox{0.8}{$\pm$0.0} \\
    \midrule
    \cmark &  & \cmark       & 12.8\scalebox{0.8}{$\pm$0.2} & 4.0\scalebox{0.8}{$\pm$0.0} \\
    \midrule
    \cmark &   \cmark     &  & 11.4\scalebox{0.8}{$\pm$0.2} & 6.8\scalebox{0.8}{$\pm$0.0} \\
    \midrule
     &  \cmark \cmark \cmark  &  & 10.8\scalebox{0.8}{$\pm$0.2} & 6.5\scalebox{0.8}{$\pm$0.0} \\
    \midrule
    \cmark & \cmark & \cmark & \textbf{9.5}\scalebox{0.8}{$\pm$0.1} & \textbf{2.5}\scalebox{0.8}{$\pm$0.0} \\
    \bottomrule
\end{tabular}}
\end{table}

==> Tables/diffusion_domain.tex <==
\begin{table}[tb]
\caption{The effectiveness of our discrete and continuous denoising scheme, in comparison to an existing discrete only representation AnalogBits and our system without the discrete branch/loss that reduces to a standard denoising scheme.
%Diversity score of using different domain for diffusion training. Can we add 2 more columns "discrete" and "continuous", and put a check mark like below?
}
\label{tab:diffusion_domain}
\centering
\setlength{\tabcolsep}{3pt}
\small
\scalebox{1.}{\begin{tabular}{c|cc|c|c}
\toprule
   & Cont. & Disc. & Divers. $(\downarrow)$ & Compat. $(\downarrow)$\\
    %
%    \cmidrule(lr){1-1}\cmidrule(lr){2-3} \cmidrule(lr){4-5}
    \cmidrule(lr){1-5}
    %
    AnalogBits~\cite{chen2022analog} & & \cmark & 14.5\scalebox{0.8}{$\pm$0.3} & 6.0\scalebox{0.8}{$\pm$0.03}\\
    \midrule
    Ours w/o disc. & \cmark &  & 38.8\scalebox{0.8}{$\pm$0.9} & 2.2\scalebox{0.8}{$\pm$0.0} \\
    \midrule
    Ours & \cmark & \cmark & 9.5\scalebox{0.8}{$\pm$0.1} & 2.5\scalebox{0.8}{$\pm$0.0} \\
    \bottomrule
\end{tabular}}
\end{table}

==> Tables/discrete_steps.tex <==
\begin{table}[tb]
\caption{\yasu{maybe, we can make this horizontal instead of vertical? I do not like the use of "Step" so many times which seem wasteful and large dead margins at the left and right.  Use abbreviation form for Diversity - Diver.   Compatibility - Compat.   Can you try making this horizontal and use double column table? We could drop 900 step case?  Typo: continues -> Continuous} Using discrete head in a few steps gives less opportunity to the network to refine the discrete coordinates, while using it early can also lead to removing necessarily continuous informations. We fix discrete head to activate when $t<32$.}
% \yasu{Maybe this is better as a bar graph or a graph instead of a table}
% \amin{Due to the scale of numbers, it's hard to show the pattern in a graph or bar, I couldn't create a good visualization yet}
\label{tab:discrete_steps}
\centering
\setlength{\tabcolsep}{3pt}
\small
\scalebox{1.}{\begin{tabular}{c|c|c}
\toprule
   Discrete steps & Diversity $(\downarrow)$ & Compatibility $(\downarrow)$\\
    %
    \cmidrule(lr){1-1}\cmidrule(lr){2-2} \cmidrule(lr){3-3}
    %
    Continues & 38.8\scalebox{0.8}{$\pm$0.9} & 2.2\scalebox{0.8}{$\pm$0.03} \\
    \midrule
    1 Step & 20.8\scalebox{0.8}{$\pm$0.3} & 3.2\scalebox{0.8}{$\pm$0.05}\\
    \midrule
    2 Step & 14.7\scalebox{0.8}{$\pm$0.6} & 3.2\scalebox{0.8}{$\pm$0.04}\\
    \midrule
    4 Step & 9.8\scalebox{0.8}{$\pm$0.2} & 3.2\scalebox{0.8}{$\pm$0.05}\\
    \midrule
    8 Step & 9.3\scalebox{0.8}{$\pm$0.2} & 3.0\scalebox{0.8}{$\pm$0.03}\\
    \midrule
    16 Step & 9.5\scalebox{0.8}{$\pm$0.1} & 2.7\scalebox{0.8}{$\pm$0.07}\\
    \midrule
    32 Step & 9.5\scalebox{0.8}{$\pm$0.1} & 2.5\scalebox{0.8}{$\pm$0.04}\\
    \midrule
    64 Step & 9.6\scalebox{0.8}{$\pm$0.2} & 2.5\scalebox{0.8}{$\pm$0.04}\\
    \midrule
    128 Step & 9.6\scalebox{0.8}{$\pm$0.1} & 2.5\scalebox{0.8}{$\pm$0.02}\\
    \midrule
    256 Step & 9.7\scalebox{0.8}{$\pm$0.3} & 2.6\scalebox{0.8}{$\pm$0.04}\\
    \midrule
    512 Step & 9.6\scalebox{0.8}{$\pm$0.2} & 2.5\scalebox{0.8}{$\pm$0.02}\\
    \midrule
    900 step & 9.8\scalebox{0.8}{$\pm$0.4} & 2.6\scalebox{0.8}{$\pm$0.05} \\
    \bottomrule
\end{tabular}}
\end{table}

==> Tables/dm_params.tex <==
\begin{table}[tb]
\caption{Results of hyper-parameter tuning on the number of steps and noise schedule for our diffusion model. We fix our experiments to 1000 steps with cosine noise schedule~\cite{nichol2021improved}.}
\label{tab:dm_params}
% \vspace{-0.9em}
\centering
\setlength{\tabcolsep}{3pt}
\small
\scalebox{.95}{\begin{tabular}{c|c|c|c}
\toprule
   Noise Schedule & Number of steps & Diversity $(\downarrow)$ & Compatibility $(\downarrow)$\\
    %
    \cmidrule(lr){1-1}\cmidrule(lr){2-2} \cmidrule(lr){3-3} \cmidrule(lr){4-4}
    %
    \multirow{1}{*}{Linear}
    & 1000 & 10.5\scalebox{0.8}{$\pm$0.1} & 2.7\scalebox{0.8}{$\pm$0.04}\\
    \midrule
    \multirow{3}{*}{Cosine}
    & 100 & 19.0\scalebox{0.8}{$\pm$0.8} & 3.1\scalebox{0.8}{$\pm$0.0}\\
    & 1000 & 9.5\scalebox{0.8}{$\pm$0.1} & 2.5\scalebox{0.8}{$\pm$0.0}\\
    & 4000 & 12.0\scalebox{0.8}{$\pm$0.3} & 3.2\scalebox{0.8}{$\pm$0.03}\\
    \bottomrule
\end{tabular}}
\end{table}

==> Tables/input_representation.tex <==
\begin{table}[tb]
\caption{The effects of the corner augmentation in the feature embedding (\ref{eq:embedding}).}
\label{tab:input_representation}
\centering
\setlength{\tabcolsep}{3pt}
\small
\begin{tabular}{c|c|c}
\toprule
   Domain & Diversity $(\downarrow)$ & Compatibility $(\downarrow)$ \\
    %
    \cmidrule(lr){1-1}\cmidrule(lr){2-2}\cmidrule(lr){3-3}
    %
    Single Corner & 10.0\scalebox{0.8}{$\pm$0.3} & 3\scalebox{0.8}{$\pm$0.0} \\
    \midrule
    Augmented Corner & 9.5\scalebox{0.8}{$\pm$0.1} & 2.5\scalebox{0.8}{$\pm$0.0} \\
    \bottomrule
\end{tabular}
\end{table}

==> Tables/main_results.tex <==
\begin{table*}[!tb]
\caption{Main quantitative results, comparing HouseDiffusion (ours) with the previous methods on the three metrics. In all experiments, our method significantly outperform all the other methods.}
%the current state-of-the-arts.}
\label{tab:main_results}
\centering
\setlength{\tabcolsep}{3pt}
\small
\begin{tabular}{c|c|c|cccc|cccc}
\toprule
   & \multicolumn{1}{c}{} & \multicolumn{1}{c}{Realism $(\uparrow)$} & \multicolumn{4}{c}{Diversity $(\downarrow)$} & \multicolumn{4}{c}{Compatibility $(\downarrow)$} \\
    %
    \cmidrule(lr){3-3}\cmidrule(lr){4-7}\cmidrule(lr){8-11} Dataset & Model &
    8 & 5 & 6 & 7 & 8 & 5 & 6 & 7 & 8 \\
    %
    \midrule
    \multirow{5}{*}{{RPLAN}} & 
    Ashual \etal~\cite{ashual2019specifying} & -1.00 & 120.6\scalebox{0.8}{$\pm$0.5} & 172.5\scalebox{0.8}{$\pm$0.2} & 162.1\scalebox{0.8}{$\pm$0.4} & 183.0\scalebox{0.8}{$\pm$0.4} & 7.5\scalebox{0.8}{$\pm$0.0} & 9.2\scalebox{0.8}{$\pm$0.0} & 10.0\scalebox{0.8}{$\pm$0.0} & 11.8\scalebox{0.8}{$\pm$0.0}\\
    %
    & Johnson \etal~\cite{johnson2018image} & -1.00 & 167.2\scalebox{0.8}{$\pm$0.3} & 168.4\scalebox{0.8}{$\pm$0.4} & 186.0\scalebox{0.8}{$\pm$0.4} & 186.0\scalebox{0.8}{$\pm$0.4} & 7.7\scalebox{0.8}{$\pm$0.0} & 6.5\scalebox{0.8}{$\pm$0.0} & 10.2\scalebox{0.8}{$\pm$0.0} & 11.3\scalebox{0.8}{$\pm$0.1}\\
    %
    & House-GAN~\cite{housegan} & -0.95 &  37.5\scalebox{0.8}{$\pm$1.1} & 41.0\scalebox{0.8}{$\pm$0.6} & 32.9\scalebox{0.8}{$\pm$1.2} & 66.4\scalebox{0.8}{$\pm$1.7} & 2.5\scalebox{0.8}{$\pm$0.1} & 2.4\scalebox{0.8}{$\pm$0.1} & 3.2\scalebox{0.8}{$\pm$0.0} & 5.3\scalebox{0.8}{$\pm$0.0}\\
    %
    & House-GAN++~\cite{houseganpp} & -0.52 & 30.4\scalebox{0.8}{$\pm$4.4} & 37.6\scalebox{0.8}{$\pm$3.0} & 27.3\scalebox{0.8}{$\pm$4.9} & 32.9\scalebox{0.8}{$\pm$4.9} & 1.9\scalebox{0.8}{$\pm$0.3} & 2.2\scalebox{0.8}{$\pm$0.3} & 2.4\scalebox{0.8}{$\pm$0.3} & 3.9\scalebox{0.8}{$\pm$0.5}\\
    %
    & Ours & \textbf{-0.19} & \textbf{11.2}\scalebox{0.8}{$\pm$0.2} & \textbf{10.3}\scalebox{0.8}{$\pm$0.2} & \textbf{10.4}\scalebox{0.8}{$\pm$0.4} & \textbf{9.5}\scalebox{0.8}{$\pm$0.1} & \textbf{1.5}\scalebox{0.8}{$\pm$0.0} & \textbf{1.2}\scalebox{0.8}{$\pm$0.0} & \textbf{1.7}\scalebox{0.8}{$\pm$0.0} & \textbf{2.5}\scalebox{0.8}{$\pm$0.0}\\
    
    \midrule
    \multirow{2}{*}{{NM-RPLAN}} &
House-GAN++~\cite{houseganpp} & --- & 77.3\scalebox{0.8}{$\pm$0.8} & 60.0\scalebox{0.8}{$\pm$0.7} & 73.8\scalebox{0.8}{$\pm$0.8} & 58.2\scalebox{0.8}{$\pm$1.0} & 1.5\scalebox{0.8}{$\pm$0.0} & 2.9\scalebox{0.8}{$\pm$0.0} & 2.1\scalebox{0.8}{$\pm$0.0} & 3.2\scalebox{0.8}{$\pm$0.0}\\
    %
& Ours & --- & \textbf{12.0}\scalebox{0.8}{$\pm$0.2} & \textbf{11.0}\scalebox{0.8}{$\pm$0.1} & \textbf{10.3}\scalebox{0.8}{$\pm$0.2} & \textbf{10.5}\scalebox{0.8}{$\pm$0.3} & \textbf{1.2}\scalebox{0.8}{$\pm$0.0} & \textbf{1.3}\scalebox{0.8}{$\pm$0.0} & \textbf{1.6}\scalebox{0.8}{$\pm$0.0} & \textbf{2.5}\scalebox{0.8}{$\pm$0.0}\\

    \bottomrule
\end{tabular}
\end{table*}

==> Tables/output_value.tex <==
\begin{table}[b]
\caption{Training the network to predict $\epsilon$ works better in our task comparing with $x_0$ as the output of the model in each step.}
\vspace{-1em}
\label{tab:output_value}
\centering
\setlength{\tabcolsep}{3pt}
\small
\scalebox{1.}{\begin{tabular}{c|c|c}
\toprule
   Network's output & Diversity $(\downarrow)$ & Compatibility $(\downarrow)$\\
    %
    \cmidrule(lr){1-1}\cmidrule(lr){2-2} \cmidrule(lr){3-3}
    %
    $x_0$ & 121.2\scalebox{0.8}{$\pm$1.9} & 4.2\scalebox{0.8}{$\pm$0.0} \\
    \midrule
    $\epsilon$ & 38.8\scalebox{0.8}{$\pm$0.9} & 2.2\scalebox{0.8}{$\pm$0.0}\\
    \bottomrule
\end{tabular}}
\end{table}
